Darks and Stripes: Effects of Clothing on Weight Perception

In many societies, appearing slim is considered attractive. The fashion industry has been attempting to cater to this trend by designing outfits that can enhance the appearance of slimness. Two anecdotal rules, widespread in the world of fashion, are (1) choose dark clothes and (2) avoid horizontal stripes, in order to appear slim. Thus far, empirical evidence has been unable to conclusively determine the validity of these rules, and there is consequently much controversy regarding the impact of both color and patterns on the visual perception of weight. In this paper, we aim to close this gap by presenting the results from a series of large-scale crowdsourcing studies that investigate the above two claims. We gathered a dataset of around 1,000 images of people from the Web together with their ground-truth weight and height, as well as clothing attributes about colors and patterns. To elicit the effects of colors and patterns, we asked crowd workers to estimate the weight in each image. For the analysis, we controlled potential confounds by matching images in pairs where the two images differ with respect to color or pattern, but are similar with respect to other relevant aspects. We created image pairs in two ways: first, observationally, i.e., from two real images; and second, experimentally, by manipulating the color or pattern of clothing in a real image via photo editing. Based on our analysis, we conclude that (1) dark clothes indeed decrease perceived weight slightly but statistically significantly, and (2) horizontal stripes have no discernible effect compared to solid light-colored clothes. These results contribute to advancing the debate around the effect of specific clothing colors and patterns and thus provide empirical grounds for everyday fashion decisions. Moreover, our work gives an outlook on the vast opportunities of using crowd sourcing in the modern fashion industry.

==> _body_BEFORE-BOBS-EDITS.tex <==
\section{Introduction}

%\todo[inline]{Add some more related work on crowdsourcing, e.g. Galton and Weber}

Modern fashion industry evolves around design of visually attractive outfits. 
To create clothes that are appealing to large groups of population, stylists try to grasp the beauty standards of their society. 
It is commonly known \cite{tovee1998} that the western female beauty standards are dominated by ``the thin ideal'', which is actually getting even slimmer with time \cite{voracek2003}. While the impact of slimness on the male beauty standards is less significant, the studies suggest that obesity can have negative impact on attractiveness \cite{maisey1999}. 
It is well established that a particular choice of clothes can make individuals appear more or less slim~\cite{frith2004clothing}. Thus, one major questions of the fashion industry is the impact of clothing on slimness and weight perception.
In this paper, we address two particularly well-known pieces of fashion advice: slimming effect of dark clothes~\cite{winakor1987effect} and the exact opposite impact of clothes with horizontal stripes~\cite{swami2012}.

The effects of dark clothes on weight perception has been well accepted, both in the fashion industry \cite{klepp2017} and the research community \cite{kremkow2014}. There is agreement that a dark object is perceived smaller compared to a light-colored object of the same size. Surprisingly, however, there are no large scale empirical studies that confirm or quantify the effect of dark clothes on our perception of someone's weight. 
%\todo[inline]{Maybe it's a too strong claim, however I didn't manage to find any solid research that proves and quantifies this effect, will try to look into it more.}
%
On the other hand, there is surprisingly lot of controversy about the effect of horizontal stripes. An obvious contradiction exists between the common agreement on negative impact of horizontal stripes on slimness \cite{feldon2000} and the predictions of the Helmholtz \cite{helmholtz1867} and Oppel-Kundt\cite{oppel,kundt} illusions, which state that horizontal stripes make rectangular shapes appear both taller and slimmer. Even recent empirical studies clearly disagree about the effect of horizontal stripes: while some claim that it increases the perceived body weight \cite{swami2012}, the others suggest that the difference between striped and solid-colored clothes is negligible \cite{thompson2011}.  A considerable drawback of these experiments is their relatively small scale (at most 100 participants rating a single person/image) that does not allow to draw generalizable conclusions.

In this work, we take a novel approach to the problem and rely on crowdsourcing to conduct a large-scale study about the impact of clothing on body-size perception. We conduct a series of experiments, in which the participating crowd-workers are shown images of people and have to estimate their weight/height or choose the person that seems heavier/taller.

Our set of images consists of a large number of photos (ca. 1,100) of people wearing various styles of clothes. 
Most images (ca. 1,000) were collected from an online weight-loss forum and were annotated with the ground truth weight and height labels by the users who uploaded them. This set of original photos was enhanced by adding 100 images edited with Adobe Photoshop in such manner that only the color (dark/light) and pattern (horizontal stripes/solid color) of the clothes were changed. Overall, we obtain the annotated image set that is unique in terms of both its size and suitability to our tasks. 

Building upon these novel datasets, we conducted three crowd sourcing experiments. 
First, for each image from a large `in the wild' dataset, we collect multiple independent weight and height guesses from crowd-workers. We then carefully match on related covariates and use the crowd responses to measure the effects of dark/light and striped clothing on the perceived weight (\Secref{sec:large}). 
Next, in the second study, we perform a similar experiment with the carefully curated edited images, thus adjusting for various potential biases that arise in the first task (\Secref{sec:clean}). 
Finally, in the last study, the images that were estimated to be similar by crowd workers are compared to each other directly. For this purpose, we compare each pair of similar images and let crowd-workers decide who of the two persons appears heavier. Using the edited images, we can compare each pair in different scenarios (e.g. one person wearing light clothes and another - dark, both wearing light, or both wearing dark) and, thus, segregate the real effect of clothing on weight or height perception (\Secref{sec:pairwise}). 

Exploiting the scalability of the crowdsourcing approach, we gathered more than 75k estimates from around 6.5k crowd-workers in the three experiments. These guesses are used to verify the impact of both color and stripes on the slimness and weight perception and, even more importantly, estimate the magnitude of these effects, thus, providing solid empirical ground for everyday fashion advice.
%
Our results provide strong evidence that (i) people do appear slimmer in dark colored clothing in comparison to light-colored or horizontally striped clothes and, (ii) wearing horizontal stripes does not necessarily make you appear fatter.
%on average, visually `reduces' the weight by ca. $2 kg$. Given the small difference, people are not very likely to notice it: if you change into dark clothes, the others are only ca. $2.5\%$ likely to notice that your body image all of a sudden appears slimmer.
%\item We settle the long on-going debate about the effects of wearing horizontal stripes~\cite{feldon2000,swami2012,thompson2011}.
%We can conclude that whether you wear light or horizontally stripped clothes, others are likely to perceive your weight in the same way.

 %The rest of the paper is organized in
%We organize the paper as follows: 
%three crowdsourcing studies --- with each study we try to build upon our previous results and, at the same time, try to address potential flaws and missing elements of the previous study. 
% We chose to organize this paper chronologically to reflect the evolution of our experimental design.
 %, as we hope that this order most accurately represents our approach and presents the steps in an easy-to-follow manner. 
 %Hence, the paper is divided into three sections each describing one of the crowdsourcing studies that we performed. 
% Section~\ref{sec:large} details the estimation of weight and height by crowd workers and the effects of clothing on a large but losely compiled dataset. Section~\ref{sec:clean} builds upon th

%\todo[inline]{write the above paragraph correctly}


\section{Data}
%Weight and height estimation with original images} 
%\subsection{Data} 
\label{subsec:large data}

The data used in this paper contains Reddit posts from weight loss forum containing posts about body weight transformation~\cite{kocabey2017face}.\footnote{\url{https://www.reddit.com/r/progresspics}} 
%The analysis in this study was performed on the set of the images \cite{kocabey2017face}. 
%The original data set contains ca. 10k samples obtained from  
%\url{https://www.reddit.com/r/progresspics} 
%forum that is dedicated to posts about body weight transformation. 
Each post contains a user's self declared height, gender, and their weight before and after the transformation, as well as one or several images showcasing their before/after transformation.\footnote{See \url{https://www.reddit.com/r/progresspics/comments/b9b53z/m3558_191lbs_to_170lbs21lbs_10_months_thx_to_all/} for an example.} 
%
To ensure high quality data, we removed posts with multiple images and ensured that each image in our set shows exactly one full-dressed person.
%performed a few additional pre-processing steps to prepare the data for our weight and height labelling task. 
%\todo[inline]{say something about the task before mentioning it}
%In particular, we ensured high quality of the data with respect to the given task: each image in our set shows exactly one full-dressed person. 
The resulting data set contains 950 images (555 female and 395 male images). A summary of the the body type classification by BMI\footnote{\url{https://www.cdc.gov/healthyweight/assessing/bmi/adult\_bmi/index.html}} is presented in \Tabref{tab:BMI data large}. 
We see that a majority of the users in our dataset are obese.
We also inspected the data set manually and characterized the different types of images present in our data. 
(i) ca. 35\% of the photos are full body pictures, the rest only contain just the torso or above, 
and, (ii) ca. 40\% of the data are selfies taken in a mirror.%, and 
Two samples from the resulting data set are shown in \Figref{fig:samples}. 
% (iii) in more than 90\% of the images we can see the head/face of the person.
% removed this to avoid complaints on privacy
 
Furthermore, 
%we obtained the pose of the person in the image 
using a state of the art pose recognition algorithm, PoseNet \cite{cao2016}, along with a few heuristics, we annotated each image with a \textit{color} attribute (dark, light, or neutral) and a flag indicating presence of \textit{horizontal stripes} in the outfit. 
The methods that we used are described below. %fully described in the Appendix \Secref{sec:color classification}-\Secref{sec:stripes detection}. 


\begin{table}
    \caption{Body type classification of the original data set from Reddit using BMI. We see that a majority of the users in our data are obese.}
    \begin{tabular}{ c | c | c | c | c | c}
    \hline
    \textbf{BMI Type} & Underweight & Normal & Overweight & Obese \\
	\hline 
	\textbf{Share, [\%]} & 0.5 & 16.7 & 25.7 & 57.1 \\
	\end{tabular}
    \label{tab:BMI data large}
\vspace{-\baselineskip}
\end{table}

\begin{figure}[t]
    \centering  
    \begin{subfigure}{.49\linewidth}
        \centering
        \includegraphics[width=\linewidth, clip=true, trim=0 260 20 150]{Plots/plot_sample1_new.pdf}
        \label{fig:sample1}
    \end{subfigure}%
    \begin{subfigure}{.49\linewidth}
        \centering
        \includegraphics[width=\linewidth, clip=true, trim=0 260 20 150]{Plots/plot_sample2_new.pdf}
        \label{fig:sample2}
    \end{subfigure}
\caption{Two samples from the dataset. Each sample contains a ``before'' and an ``after'' picture.}
\label{fig:samples}
\end{figure}

\subsection{Color classification} \label{sec:color classification}

As the first step to estimation of the impact of clothes color on weight perception, a systematic way to classify the clothes as dark- or light-colored (or possibly neutral) is required. In this section, we describe our approach that avoids tedious and, possibly, biased manual inspection.
%
When referring to the color or stripes in the clothing, we refer only to the upper-body clothing. 
This is not a weak assumption since we are interested in weight perception, and the upper body plays a significantly important role in this. 
This formulation also fits particularly well to the data set at hand because of many images that show only a person's torso and not their full body.   

Our approach to color detection relies on the PoseNet \cite{cao2016} for body pose recognition. 
PoseNet, given an image, identifies the approximate pose by identifying all joints and body parts.
Once the positions of all joints and body parts are localized, we can sample the $RGB$-values (in range $[0, 255]$) of the pixels along the main upper body line - from the neck to the underbelly. 
We define the resulting color of the outfit as the value mean of the three channels of all sampled pixels. 
In this way, every image can be assigned a single `brightness value' $bv$ with $0$ being perfect black and $255$ perfect white. 

We used the described algorithm to compute brightness values $bv$ for all images in the image set from Section \ref{subsec:large data}. We manually evaluated the algorithm on all a sample of 100 images in the dataset and it works perfectly. 
Fig. \ref{fig:color qunatiles} shows 4 sample images with the corresponding values $bv$.

\begin{figure}[ht]
  \centering
  \includegraphics[width=0.45\textwidth]{Plots/color_quantiles.pdf}
  \caption{Sample images with detected body line and computed brightness value ($bv$). The images are (from left to right) at 0th (the darkest), 33th, 66th and 100th (the brightest) percentile of $bv$.}
  \label{fig:color qunatiles}
\end{figure}


\subsection{Stripes detection} \label{sec:stripes detection}

To make grounded statements on the effect of horizontal stripes on slimness, a large number of samples with striped clothing is required. 
A relatively small size of the image set from \Secref{subsec:large data} lets us detect the relevant samples manually. However, it turns out that wearing horizontal stripes is rather uncommon (from  images from \Secref{subsec:large data} only ca. 35 are suitable). Thus, an automated approach for collection and processing of additional data is required.

Similar to the color classification in \Secref{sec:color classification}, our approach for stripes detection relies on the PoseNet for detection of the main upper body line. $RGB$ values are sampled along the detected line and a single value for each pixel is computed by averaging over three color channels. Then we process the sequence of sampled pixel-wise values by a median (of length 5) and a third-order Savgol filter, which smoothes the noise and undesired fluctuations. 
Finally, we apply a Fourier transform on the output of the filters. The amplitudes of the resulting Fourier coefficients of different frequencies are important: our experiments suggest that stripes on the clothes lead to a large coefficient of the frequency that corresponds to the actual number of visible stripes. 
Therefore, we make use of the following heuristic rule: classify as a positive example (striped) any outfit that has its maximal (in terms of amplitude) Fourier coefficient in the range $[6,25]$, corresponding to a typical number of visible stripes. 
\Figref{fig:stripes classifier} illustrates the method on an image that is classified as positive.

\begin{figure*}
\centering
\begin{subfigure}{.24\textwidth}
  \centering
  \includegraphics[width=0.4\linewidth, clip=true, trim=50 10 100 10]{Plots/plot_stripes_sample.png}
  \caption{}
\end{subfigure}%
\begin{subfigure}{.24\textwidth}
  \centering
  \includegraphics[width=\linewidth]{Plots/plot_stripes_colorline.pdf}
  \caption{}
\end{subfigure}
\begin{subfigure}{.25\textwidth}
  \centering
  \includegraphics[width=\linewidth]{Plots/plot_stripes_colorline_smooth.pdf}
  \caption{}
\end{subfigure}
\begin{subfigure}{.25\textwidth}
  \centering
  \includegraphics[width=\linewidth]{Plots/plot_stripes_colorline_fourier.pdf}
  \caption{}
\end{subfigure}
\caption{Steps of the algorithm for stripes detection: identification of the main upper-body line (a), pixel-wise sampling of RGB values (mean subtracted) along the line (b), application of smoothing filters to the pixel-wise RGB values (c), and Fourier transform of the resulting sequence (d). The sample is classified as positive because of the magnitude of the 19-th Fourier coefficient (note that exactly 19 stripes are crossed by the main body line).}
\label{fig:stripes classifier}
\end{figure*}

We should point out that the resulting algorithm relies on empirical observation and heuristics, so that the obtained results are far from perfect. In many cases other periodic variations of color (e.g. checkerboard patterns, letters, graphics or just different shading due to certain light conditions) trigger a positive response. Overall only ca. 20\% of the detected samples indeed wear horizontal stripes, and thus, manual inspection of the results is required to remove false positives. 
Nevertheless, the algorithm performs well for our purposes, as it provides a fast and simple way to detect striped clothes at scale. With this method we processed a dataset of over 30,000 images from Reddit posts and obtained 90 images of people wearing clothes with horizontal stripes to the data set. 

\section{Crowdsourcing the estimation of weight and height} 
\label{subsec:large crowdsourcing}
In this section, we describe the setting of our crowd sourcing efforts to collect height and weight estimates. 
Note that though we are only interested in the effects of clothing on perceived weight, as a simple side effect of the crowd sourcing data collection, we also collect the perceived height data.
Since height perception should not change significantly depending on clothing, we can use these estimates to validate our experimental setup and data collection.
%our first study to estimate the effect of clothes on weight perception. 

%To obtain estimates on the \textit{perceived} weight and height by others, we use crowd sourcing.

%We begin by 
%\todo[inline]{write properly. describe exactly whats being done}

%To measure how well humans are at estimating height and weight from images, we setup a 
We use Amazon Mechanical Turk to gather weight and height estimates from a diverse pool of crowd workers. 
We divided the set of images in our dataset into tasks with 10 images each. For each image, crowd workers had to guess the weight and height of the shown person. Two corresponding input fields were located under the image, with the field for weight guesses coming first. 
We aimed to provide familiar units for a possibly large pool of crowd-workers and gave a choice between ``kg'' and ``lbs'' units for weight estimation, and ``cm'' and ``ft/in'' for height estimation. 
To avoid confusions, automatic conversions between different units were performed on the fly, i.e., the other field was updated at the same time as workers were typing the guesses in their preferred format. 
%For this experiment, the base reward amounted to 1 cent per image. 
Finally, we encouraged high-quality estimates by awarding 25\% of the most accurate (on per task basis) workers with a large bonus that would double their usual payment.

%of the people captured in these images. 
%In the initial design of the experiment, the crowd workers did not receive any feedback about their accuracy and did not have access to the previously collected guesses of other workers. 
In this way, we collected 45 weight and height labels for each image, which amounts to more than 42k estimates from 3.5k unique workers. We filtered and preprocessed the collected raw weight and height estimates by removing guesses from workers who appear to have used scripts to generate random values, and erroneous guesses, such as typos or usage of wrong measurement units (e.g. a worker accidentally chose ``kg'' and ``lbs'' or vice versa).
After these processing steps, we were left with roughly 80\% of the initial estimates.% remained in each of the sets.

 %Sections~\ref{sec:gen accuracy}--\ref{sec:correction} focus mostly on this main data set. 


%\subsection{Analysis}%Aggregation of estimates}
%Methods of analysis} 
%\label{subsec:large analysis}
%In the following, we describe the approach for aggregation of multiple guesses by crowd workers to per-image estimates, and discuss the methods and metrics used for analysis and comparison of the resulting per-image estimates. 

\xhdr{Aggregation of estimates}
We obtain 45 estimates per image. To obtain a single estimate, one possible approach to leverage the `wisdom of the crowds' is to compute the mean of all collected guesses as an estimate of the true weight $w^i_\true$ for an image $i$: 
\begin{equation}
	w_{\est}^i =  \frac{1}{n} \sum_{j=1}^{n} w_{j}^i,
\end{equation}
where $w_1^i,\dots,w_n^i$ are the weight guesses of individual workers for image $i$. Similarly, for the image $i$ we denote the true height, $h^i_{\true}$, and the estimated height, $h^i_{\est}$.\footnote{For readability, we henceforth drop the image index $i$ when no confusion can arise.} Based on the known, self reported $w_\true$ and $h_\true$ (or $w_\est$ and $h_\est$) we can calculate the true BMI, $BMI_{\true}$ (or the estimated $BMI_{\est}$), for all images. Note that the $BMI$ values $BMI_\est$ are computed from the collected (and averaged) guesses of weight and height, and not estimated directly by the crowdworkers.   

Our approach is slightly different from the original wisdom of the crowds idea of Francis Galton \cite{galton1907vox} who suggested to use the median (instead of mean) of all collected guesses as a single estimate. 
Our experiments showed that the difference between both methods for the considered task is negligible. Given their similar accuracy, we use the mean value as the aggregate estimate in the rest of the paper.

\Figref{fig:convergence} shows the dependence of the mean weight error on the number of collected guesses for two sample images. To produce these plots, we collected 75 guesses for a few images and observed the convergence behavior of the resulting estimates. The convergence rate of the aggregated estimates quickly drops after around 30 guesses. Thus, \Figref{fig:convergence} post-hoc justifies our choice of 45 guesses as the lower bound on the number of collected estimates per image. 

\begin{figure}
    \centering
	\begin{subfigure}{.24\textwidth}
 		\centering
  		\includegraphics[width=\linewidth]{Plots/plot_convergence_1.pdf}
	\end{subfigure}%
	\begin{subfigure}{.25\textwidth}
  		\centering
  		\includegraphics[width=\linewidth]{Plots/plot_convergence_2.pdf}
  	\end{subfigure}
	\caption{Average of all weight guesses for two sample images with 95\% confidence intervals, in dependence of the number of collected estimates (computed from 1,000 random simulation in which guesses come in different order).}
	\label{fig:convergence}
\end{figure}


\section{Study1: Comparison of perceived weight}% on the Large dataset}
\label{sec:large}

In this section, we study the effects of change in weight perception on the large dataset of ca. 1000 images described in \Secref{subsec:large data}. We do this by carefully matching images which are similar to each other in terms of various related covariates.

%\xhdr{Matching}
%
Previous research on visual weight and height estimation \cite{cornelissen2016visual} 
suggests that the gender, and, especially, the true body measurements of people shown in the images strongly correlate with the errors on the aggregated estimates. Particularly, heavier users are consistently under estimated and light weight people are over estimated.  

Given these biases in human perception, we have to match the populations of people wearing different types of clothes in order to properly evaluate the effect of clothing change. 
In our data set, only three measured covariates are available: gender of the person, their true weight and height. Since the space of covariates is low dimensional (one binary and two contnuous variables), direct matching of covariates leads to accurate results and even outperforms more sophisticated methods, such as propensity score matching. 
Thus, we consider a pair of images to be a valid candidate for matching if:
\begin{itemize}
    \item both persons wear different types clothes,
    \item their true weight and height differ at most by $t_w$ kg and $t_h$ cm respectively,
    \item their true BMI difference is below 1 point, which is the so-called just noticeable difference \cite{cornelissen2016visual} (the BMI difference that people can not consistently detect).
\end{itemize}
The thresholds $t_w$ and $t_h$ ensure that the individual images within each pair are close to each other. 

The above condition can be modeled as a bipartite graph where a valid candidate pair of images is connected by an edge. To find the largest possible (in terms of the number of pairs) matching, we perform a maximum matching algorithm on the resulting graph.

\textit{Remark:} As previously discussed, there are multiple others attributes that contribute to the weight/height estimation process. However, most of these characteristics are purely visual, e.g. pose, camera angle or background, and, thus, can hardly be measured and matched. 

\xhdr{Metric} 
After matching two populations, we consider the \textit{pairwise difference of estimates}. For a matched pair $i$ that contains one image from the first group, $i_1$, and one image from the second group, $i_2$, we define this quantity as:
\begin{equation}
    \Delta w^i_\est = w^{i_1}_\est - w^{i_2}_\est, \label{eqn:pairwise difference}
\end{equation}
and similarly for $\Delta h^i,\ \Delta BMI^i$. Whenever the difference in clothes has no impact on the perceived weight (or height, or BMI), we expect a zero-centered distribution of the pairwise differences, given the previously matched populations. On the other hand, if the distribution of pairwise differences is skewed, we can assume that a certain type of clothing has a slimming or fattening effect.  

\subsection{Results} \label{subsec:large results}

%In the following, we summarize the study results. 
For the matching, we use the threshold values of $t_w = 2.5 kg$ and $t_h = 2.5 cm$. Clearly, there exists a trade-off between the number of matching pairs and the quality of the resulting matching, and we can influence this trade-off by adjusting the threshold values. Our experiments show that the results are robust with respect to these values. We believe that the chosen thresholds are reasonable as they ensure an accurate matching within single pairs and still lead to sufficiently large data sets. 
The distributions of difference between covariates in the matched pairs for various types of images (described below) are summarized in \Tabref{tab:matching}.  

\begin{table}[]
    \caption{Results of matching on the different sets of images: mean differences among pairs and $p-$values of the Wilcoxon's test for weight, height and BMI. Note that the height is equal within each pair because the original data had height labels in inches and one inch exceeds the chosen threshold.}
    \label{tab:matching}
    \centering
    \begin{tabular}{l|c|c|c}
        Metric & Dark/Light & Light/Striped & Dark/Striped \\
        \hline
        Number of pairs & 153 & 65 & 54 \\
        Mean weight difference & -0.04 & -0.13 & -0.30 \\
        $p$-value for weight & 0.71 & 0.60 & 0.16 \\
        Mean height difference & 0 & 0 & 0 \\
        Mean BMI difference & -0.02 & -0.04 & -0.10 \\
        $p$-value for BMI & 0.67 & 0.63 & 0.19 \\
    \end{tabular}
\end{table}

\xhdr{Effect of clothing color}
We begin by considering the impact of the clothing color on weight perception. 
For this purpose, we exclude the images that contain horizontal stripes and split all remaining samples into three equally-sized groups based on the computed color attribute, $bv$ (cf. \Secref{sec:color classification}), of the clothes: dark- (lower third of $bv$ values), light- (upper third of $bv$) and neutral-colored (rest). Here, we compare the groups of dark- and light-colored images. 
The chosen thresholds lead to 153 (out of almost 300 possible) valid dark- and light-colored pairs. 

%To be precise with the definition (\ref{eqn:pairwise difference}), let the populations of images with dark and light clothes be groups 1 and 2, respectively. 
The distributions of $\Delta w_\est, \Delta h_\est, \Delta BMI_\est$ for images with dark and light clothes are shown in \Figref{fig:dist w dirty dl}-\Figref{fig:dist bmi dirty dl}. 
More detailed results, showing individual pairs, can be seen in the scatter plots in \Figref{fig:scatter w dirty dl}-\Figref{fig:scatter bmi dirty dl} where each point depicts a single pair of images. 
The distributions of $\Delta w_\est$ and $\Delta BMI_\est$ in \Figref{fig:dist w dirty dl} and \Figref{fig:dist bmi dirty dl} are clearly left-skewed, and thus indicate that people wearing dark are, on average, perceived as being lighter and slimmer (whether and how accurately BMI can assess slimness is controversial, but it is widely accepted as an indicator of healthy weight, and we will use it here and in the following as a measure related to slimness). 
Similar conclusion can be drawn from \Figref{fig:scatter w dirty dl} and \Figref{fig:scatter bmi dirty dl} where the majority of points lies above the diagonal (thus, indicating that the light-colored samples are mostly estimated heavier and less slim). For comparison, the centered distribution of $\Delta h_\est$ in \Figref{fig:dist h dirty dl} and a relatively balanced `diagonal' plot of pairs in \Figref{fig:scatter h dirty dl} demonstrate that the height guesses were not affected by the color of the clothes. 

The above results are supported by the statistics provided in \Tabref{tab:dirty set summary} that contain the values of the average differences in estimated measurements between both groups, as well as the $p-$values of the Wilcoxon's test that we performed on the populations after matching.

\begin{figure}
    \centering
	\begin{subfigure}{.33\columnwidth}
 		\centering
  		\includegraphics[width=\linewidth]{Plots/plot_dist_w_pairwise_est_dirty_dl.pdf}
  		\caption{} \label{fig:dist w dirty dl}
	\end{subfigure}%
	\begin{subfigure}{.33\columnwidth}
  		\centering
  		\includegraphics[width=\linewidth]{Plots/plot_dist_h_pairwise_est_dirty_dl.pdf}
  		\caption{} \label{fig:dist h dirty dl}
  	\end{subfigure}
	\begin{subfigure}{.33\columnwidth}
  		\centering
  		\includegraphics[width=\linewidth]{Plots/plot_dist_bmi_pairwise_est_dirty_dl.pdf}
  		\caption{} \label{fig:dist bmi dirty dl}
  	\end{subfigure}
	\caption{Distributions of pairwise differences of estimated weight (left), height (center) and BMI (right).}% for people wearing dark-colored (group 1) and light-colored (group 2) clothes.}
  	\label{fig:dist dirty dl}
\end{figure}
	
\begin{figure}
    \centering
	\begin{subfigure}{.33\columnwidth}
 		\centering
  		\includegraphics[width=\linewidth, clip=true, trim=40 10 60 10]{Plots/plot_scatter_w_pairwise_comp_dirty_dl.pdf}
  		\caption{} \label{fig:scatter w dirty dl}
	\end{subfigure}%
	\begin{subfigure}{.33\columnwidth}
  		\centering
  		\includegraphics[width=\linewidth, clip=true, trim=40 10 60 10]{Plots/plot_scatter_h_pairwise_comp_dirty_dl.pdf}
  		\caption{} \label{fig:scatter h dirty dl}
  	\end{subfigure}
	\begin{subfigure}{.33\columnwidth}
  		\centering
  		\includegraphics[width=\linewidth, clip=true, trim=40 10 60 10]{Plots/plot_scatter_bmi_pairwise_comp_dirty_dl.pdf}
  		\caption{} \label{fig:scatter bmi dirty dl}
 	\end{subfigure}
 	\caption{Scatter plots with pairs of weight (left), height (center) and BMI (right) estimates. $x-$ and $y-$coordinates denote the resulting estimates of measurements for people wearing dark- and light-colored clothes respectively. Dashed line denotes the equal estimates, i.e. $w^{i_1}_\est == w^{i_2}_\est$.}
 	\label{fig:scatter dirty dl}
\end{figure}

\xhdr{Effect of striped clothing}
We conducted similar analysis to test the second hypothesis: the fattening effect of outfits with horizontal stripes, and compared the striped clothes (group 1) with both light- and dark-colored outfits (group 2). 
We perform the matching of pairs with the same threshold parameters as before, leading to 65 and 54 pairs of (light, striped) and (dark, striped) clothes respectively. 
For the space reasons, we only provide the distribution and scatter plots that show the comparison of striped- and light-colored clothes. The statistical results in \Tabref{tab:dirty set summary} cover all cases.

Like above, Figures \Figref{fig:dist w dirty ls}-\Figref{fig:dist bmi dirty ls} show the distribution of $\Delta w_\est, \Delta h_\est, \Delta BMI_\est$. The centered distributions in \Figref{fig:dist w dirty ls}-\Figref{fig:dist bmi dirty ls} as well as the scatter plots centered around the diagonal in \Figref{fig:scatter w dirty ls}-\Figref{fig:scatter bmi dirty ls} indicate that horizontal stripes do not have any negative effect on weight, height or slimness when compared to the light-colored outfits. 
This conclusion is further supported by the results of statistical tests in \Tabref{tab:dirty set summary}. 

\begin{figure}
    \centering
	\begin{subfigure}{.33\columnwidth}
 		\centering
  		\includegraphics[width=\linewidth]{Plots/plot_dist_w_pairwise_est_dirty_ls.pdf}
  		\caption{} \label{fig:dist w dirty ls}
	\end{subfigure}%
	\begin{subfigure}{.33\columnwidth}
  		\centering
  		\includegraphics[width=\linewidth]{Plots/plot_dist_h_pairwise_est_dirty_ls.pdf}
  		\caption{} \label{fig:dist h dirty ls}
  	\end{subfigure}
	\begin{subfigure}{.33\columnwidth}
  		\centering
  		\includegraphics[width=\linewidth]{Plots/plot_dist_bmi_pairwise_est_dirty_ls.pdf}
  		\caption{} \label{fig:dist bmi dirty ls}
  	\end{subfigure}
  	  \caption{Distributions of pairwise differences of weight (left), height (center) and BMI (right) for people wearing light-colored (group 1) and horizontally striped (group 2) clothes.}
\end{figure}
	
\begin{figure}
    \centering
	\begin{subfigure}{.33\columnwidth}
 		\centering
  		\includegraphics[width=\linewidth, clip=true, trim=40 10 60 10]{Plots/plot_scatter_w_pairwise_comp_dirty_ls.pdf}
  		\caption{} \label{fig:scatter w dirty ls}
	\end{subfigure}%
	\begin{subfigure}{.33\columnwidth}
  		\centering
  		\includegraphics[width=\linewidth, clip=true, trim=40 10 60 10]{Plots/plot_scatter_h_pairwise_comp_dirty_ls.pdf}
  		\caption{} \label{fig:scatter h dirty ls}
  	\end{subfigure}
	\begin{subfigure}{.33\columnwidth}
  		\centering
  		\includegraphics[width=\linewidth, clip=true, trim=40 10 60 10]{Plots/plot_scatter_bmi_pairwise_comp_dirty_ls.pdf}
  		\caption{} \label{fig:scatter bmi dirty ls}
 	\end{subfigure}
 	 \caption{Scatter plots with pairs of weight (left), height (center) and BMI (right) estimates. $x-$ and $y-$coordinates denote the resulting estimates of measurements for people wearing light-colored and horizontally striped clothes respectively. Dashed line denotes the equal estimates, i.e. $w^{i_1}_\est = w^{i_2}_\est$.}
\end{figure}

On the other hand, the dark clothes show a clear difference in comparison against horizontal stripes (\Tabref{tab:dirty set summary}), indicating that dark clothing makes you appear slimmer compared to horizontal stripes.%and, once again, demonstrate positive influence on visual slimness.

\begin{table*}
	\caption{Summary of results on the set of original images: comparison of estimated weight, height and BMI for different groups after matching the populations (according to definition (\ref{eqn:pairwise difference}) the format in the top row is group1/group2). Mean pairwise difference of estimated measurements (with 95\% confidence intervals) and $p-$values of Wilcoxon's test.}
	\centering
    \begin{tabular}{l|c|c|c}
        Metric & Dark/Light & Light/Striped & Dark/Striped \\
        \hline
        Number of pairs & 153 & 65 & 54 \\
        \hline
        Weight est.: mean difference & -2.27 (-3.74,-0.83) & -0.18 (-2.54,2.09) & -3.08 (-5.38,-0.77) \\
        Weight est.: $p$-value & 0.004 & 0.68 & 0.007 \\
        \hline
        Height est.: mean difference of  & -0.11 (-0.77,0.55) & -0.21 (-1.05,0.64) & -0.01 (-0.97,0.98) \\
        Height est.: $p$-value & 0.88 & 0.56 & 0.79 \\
        \hline
        BMI est.: mean difference & -0.77 (-1.24,-0.31) & 0.06 (-0.69,0.77) & -1.05 (-1.74,-0.34) \\
        BMI est.: $p$-value & 0.002 & 0.70 & 0.007 \\
    \end{tabular}
    \label{tab:dirty set summary}
\end{table*}

Overall, the conclusion from the crowdsourcing study in this section and the results in Table~\ref{tab:dirty set summary} can be summarized by the following two statements:
\begin{itemize}
    \item dark clothes show a small but statistically significant effect on the perceived weight: on average, the weight of people wearing dark is estimated to be 2 to 3 kg less when compared with the similar people wearing light colors or horizontal stripes,
    \item the outfits with horizontal stripes do not indicate any significant difference on the perceived body measurements when compared to the light-colored clothes. 
\end{itemize}


\section{Study2: Comparison of perceived weight with edited images} 
\label{sec:clean}

The analysis presented in \Secref{sec:large} relied on matching of different populations with respect to their real weight and height. 
While this procedure eliminates a large source of possible biases, it by no means guarantees that the resulting groups are indeed comparable. 
Image features as the face shape, body pose, camera angle, size and fit of the clothes, background color, etc., are all likely to affect the final weight guesses of crowd-workers. 
Clearly, it is impossible to take into account or even estimate all these complex factors, and we can only hope that these effects balance out on the population level. 
Apart from such rather random fluctuations, one could think of a systematic difference, e.g. what if people that already look slim also tend to choose dark clothes in order to emphasize their slimness, or vice versa, full-figured individuals prefer dark to give a slimmer image of themselves? 

%While we are not able to take into account such factors, w
We can imagine a perfect data set that would let us avoid such factors them altogether: a single sample from this ideal data set would include three images of the same person - one in light-colored clothes, one in dark, and one wearing horizontal stripes. Three images of each person would be taken under the same conditions, and the three types of clothes would differ only by their color/pattern but have the same size and fit. In this way, all undesirable and hard to measure factors would be eliminated, or at least drastically reduced, and the results on such a `clean' set would be attributed solely to the impact of the color change (or horizontal stripes). 
%
Creating such an ideal dataset of real images would require a considerable investment. 
%are required to get real images under such conditions. 
Therefore, we decided to `mock' the desired set by using graphical design on the original images. 
For this purpose, we chose 100 photos of people wearing horizontal stripes and hired an expert from an online service Fiverr\footnote{\url{https://www.fiverr.com}} to perform the following tasks in Adobe Photoshop:
\begin{itemize}
    \item remove stripes from clothing,
    \item change the color of the resulting clothes to create solid-colored dark and light versions.
\end{itemize}

\begin{figure*}
\centering
\begin{subfigure}{.15\textwidth}
  \centering
  \includegraphics[width=\linewidth]{Plots/photoshop_1.jpg}
  \caption{}
\end{subfigure}%
\begin{subfigure}{.15\textwidth}
  \centering
  \includegraphics[width=\linewidth]{Plots/photoshop_1_dark.jpg}
  \caption{}
\end{subfigure}
\begin{subfigure}{.15\textwidth}
  \centering
  \includegraphics[width=\linewidth]{Plots/photoshop_1_light.jpg}
  \caption{}
\end{subfigure}
\begin{subfigure}{.15\textwidth}
  \centering
  \includegraphics[width=\linewidth]{Plots/photoshop_2.jpg}
  \caption{}
\end{subfigure}%
\begin{subfigure}{.15\textwidth}
  \centering
  \includegraphics[width=\linewidth]{Plots/photoshop_2_dark.jpg}
  \caption{}
\end{subfigure}
\begin{subfigure}{.15\textwidth}
  \centering
  \includegraphics[width=\linewidth]{Plots/photoshop_2_light.jpg}
  \caption{}
\end{subfigure}
\caption{Two samples from the `clean' image set. We start with original photos with striped clothes, (a) and (d), and edited them to obtain solid dark-colored clothing, (b) and (e), and light-colored clothing, (c) and (e). All images of the left sample appear realistic, while the low quality of the right source image makes the edited photos look slightly artificial.}
\label{fig:photoshop}
\end{figure*}

Two examples from the resulting `clean' image set are shown in \Figref{fig:photoshop}. 
We observe that the realistic look of the obtained images strongly depends on the quality of the source photos. 
We manually ensured that most images in the data set are much closer to the original image.
%realistic sample in the left part of \Figref{fig:photoshop} than to the less convincing image shown on the right in \Figref{fig:photoshop}. 
While a photoshop expert could probably identify the edited images, we believe that the difference is hardly noticeable for most people, especially in the context of our task of height and weight estimation, for which most crowd-workers spend only a few seconds on each image. An anonymized dataset of all the 100 original and photoshopped images will be made available upon the acceptance of the paper.
%
A summary of the the body type classification by BMI for the new set is presented in Table~\ref{tab:BMI data clean}. 

\begin{table}
	\caption{Body type classification (BMI) of the set with edited images. Again, a majority of the users in the data are obese.}
    \label{tab:BMI data clean}
    \begin{tabular}{ c | c | c | c | c | c}
    \hline
    \textbf{BMI Type} & Underweight & Normal & Overweight & Obese \\
	\hline 
	\textbf{Share, [\%]} & 1 & 15 & 24 & 60 \\
	\end{tabular}
\vspace{-\baselineskip}
\end{table}


%\subsection{Crowdsourcing} \label{subsec:clean crowdsourcing}

Next, we collected weight and height estimates for the new, edited images data set, using the same study settings as discussed in \Secref{sec:large}. 
%The only differences to the previous experiment were:
In addition, in order to improve the labelling accuracy, we restricted the pool of valid workers to the residents of the US to avoid possible confounds, such as country-specific biases for estimation of weight and height. % that we discovered in our recent studies.
%\begin{itemize}
%    \item the number of collected guesses: each image from the new set was labelled by 65-75 crowd workers (compared to 45 estimates in \Secref{sec:large}), 
%    \item the demographics of the crowd workers: we restricted the pool of valid workers to the residents of the US to avoid possible confounds, such as country-specific biases for estimation of weight and height. % that we discovered in our recent studies.
%\end{itemize}

%These changes were introduced to improve the accuracy during the labelling phase, which is especially important for the `clean' set as we use it as a base for the last study described in \Secref{sec:pairwise}.
 
\subsection{Results} \label{subsec:clean results}

\iffalse
\begin{itemize}
	\item dark is slightly better than stripes and light
	\item stripes and light are similar
	\item difference in \textbf{height perception}? (striped are estimated smaller)
	\item no difference among BMI groups
\end{itemize}
\fi

%To analyze the results, we proceed similarly to \Secref{subsec:large analysis}. 
We perform our analysis similar to \Secref{sec:large}. Note that this time the matching step is not required because the exact same images are contained in all three groups (dark, light and striped).
%which is the whole point of introducing the new data set). 
Instead, we apply an additional post-hoc condition: drop all pairs where the estimated difference exceeds $10 kg$ or $10 cm$. Such pairs are likely to be corrupted by the Phothsop editing as the effect of clothes can hardly reach such extent. Indeed, visual inspection of such pairs showed that the edited images did not preserve the body silhouettes.  

We begin by comparing the dark (group 1) and light (group 2) clothes. Note how this time the images in each pair appear much more similar to the crowd workers: as expected, the variances of the distributions in \Figref{fig:dist clean dl} and deviations of the points in \Figref{fig:scatter clean dl} are much smaller compared to \Figref{fig:dist dirty dl}-\Figref{fig:scatter dirty dl}. Surprisingly however, the results depicted in \Figref{fig:dist clean dl}-\Figref{fig:scatter clean dl} and summarized in \Tabref{tab:clean set summary} indicate that there is no significant differences among \textit{all} measurements between both groups. 

\begin{figure}
    \centering
	\begin{subfigure}{.33\columnwidth}
 		\centering
  		\includegraphics[width=\linewidth]{Plots/plot_dist_w_pairwise_est_clean_dl.pdf}
  		\caption{} \label{fig:dist w clean dl}
	\end{subfigure}%
	\begin{subfigure}{.33\columnwidth}
  		\centering
  		\includegraphics[width=\linewidth]{Plots/plot_dist_h_pairwise_est_clean_dl.pdf}
  		\caption{} \label{fig:dist h clean dl}
  	\end{subfigure}
	\begin{subfigure}{.33\columnwidth}
  		\centering
  		\includegraphics[width=\linewidth]{Plots/plot_dist_bmi_pairwise_est_clean_dl.pdf}
  		\caption{} \label{fig:dist bmi clean dl}
  	\end{subfigure}
  	\caption{Edited images: distributions of pairwise differences of weight (left), height (center) and BMI (right) for people wearing dark-colored (group 1) and light-colored (group 2) clothes.} \label{fig:dist clean dl}
\end{figure}

\begin{figure}
    \centering
	\begin{subfigure}{.33\columnwidth}
 		\centering
  		\includegraphics[width=\linewidth, clip=true, trim=40 10 60 10]{Plots/plot_scatter_w_pairwise_comp_clean_dl.pdf}
  		\caption{} \label{fig:scatter w clean dl}
	\end{subfigure}%
	\begin{subfigure}{.33\columnwidth}
  		\centering
  		\includegraphics[width=\linewidth, clip=true, trim=40 10 60 10]{Plots/plot_scatter_h_pairwise_comp_clean_dl.pdf}
  		\caption{} \label{fig:scatter h clean dl}
  	\end{subfigure}
	\begin{subfigure}{.33\columnwidth}
  		\centering
  		\includegraphics[width=\linewidth, clip=true, trim=40 10 60 10]{Plots/plot_scatter_bmi_pairwise_comp_clean_dl.pdf}
  		\caption{} \label{fig:scatter bmi clean dl}
 	\end{subfigure}
 	\caption{Edited images: scatter plots with pairs of weight (left), height (center) and BMI (right) estimates from the 'clean' set. $x-$ and $y-$coordinates denote the resulting estimates of measurements for people wearing \textbf{exactly the same} dark- and light-colored clothes respectively. Dashed line denotes the equal estimates, i.e. $w^{i_1}_\est == w^{i_2}_\est$.}
 	\label{fig:scatter clean dl}
\end{figure}


For space reasons, we omit the plots for two other comparisons - between the light-colored and horizontally striped clothes, as well as between the dark and striped outfits - and provide a summary of all experiments in \Tabref{tab:clean set summary}. These results are disappointing, while the main trends - a slight slimming effect of the dark clothes and equality of the striped and light-colored outfits - that we observed on the data from \Secref{sec:large} hold, for the new set the difference between all groups is below statistical thresholds. However, we can not conclude if these differences are due to small sample sizes or due to inherent lack of any signal. 

\begin{table*}[th!]
	\centering
	\caption{Summary of results on set of edited images: comparison of estimated weight, height and BMI for different groups (according to definition (\ref{eqn:pairwise difference}) the format in the top row is group1/group2). Mean pairwise difference of estimated measurements (with 95\% confidence intervals) and $p-$values of Wilcoxon's test.}
    \begin{tabular}{l|c|c|c}
        Metric & Dark/Light & Light/Striped & Dark/Striped \\
        \hline
        Number of pairs & 98 & 99 & 97 \\
        \hline
        Weight est.: mean difference & -0.23 (-0.93,0.46) & -0.12 (-0.80,0.55) & -0.13 (-0.80,0.54) \\
        Weight est.: $p$-value & 0.34 & 0.78 & 0.50 \\
        \hline
        Height est.: mean difference of  & 0.09 (-0.20,0.37) & 0.22 (0.05,0.50) & 0.29 (0.01,0.56) \\
        Height est.: $p$-value & 0.58 & 0.09 & 0.05 \\
        \hline
        BMI est.: mean difference & -0.13 (-0.37,0.11) & -0.12 (-0.35,0.11) & 0.17 (-0.40,0.06) \\
        BMI est.: $p$-value & 0.15 & 0.50 & 0.06 \\
    \end{tabular}
    \label{tab:clean set summary}
\end{table*}


\textit{Remark}: From \Tabref{tab:clean set summary}, it appears that the strongest effect present is the difference of height estimates among striped and solid-colored samples. We designed and conducted an experiment similar to the one described in \Secref{sec:pairwise}, but did not discover any further support for this hypothesis. We believe that it is an artifact caused by the limited amount of data at hand. 

\section{Study3: Pairwise comparison of matched samples}
\label{sec:pairwise}

%\todo[inline]{Can we find any reference to support the claim that people are better when comparing two things than separately estimating each?}
In the two studies detailed in previous sections, we aimed to collect absolute estimates of weight and height for an image.
Providing an absolute estimate is a hard task, and our recent research (citation anonymized for double blind review) indicates that the results can be strongly affected by the personal biases of the crowd workers. 
%In particular, we found that even after aggregation of multiple guesses, the error for most images exceeds $5 kg$. 
We saw that the estimated measurements for different groups of the edited images (cf. \Figref{fig:scatter clean dl}) lie so close to each other that even smaller uncertainty or inaccuracy in the estimation could make our conclusions unreliable. 
%and given the weak results in \Secref{sec:clean}, 
Taking these biases into account, we designed a new study that would rely on relative comparisons between images and provide additional clarity on our previous observations. 
Providing relative comparisons has been shown to be a much easier task than absolute estimates in many psychological studies~\cite{tversky1981framing}.

%We consider the labelled images from \Secref{sec:clean} and pair them up based on their estimated weight.
Our main idea for this study is to assign the images from \Secref{sec:clean} into pairs based on their estimated weight and height (rather than on their true measurements), thus ensuring that both images in each pair \textit{appear} similar. We then let the crowd workers decide which of the two person in each image weighs less. 
Making use of the triplets (dark, light and striped versions of each image) in the data set, we can show each pair in multiple configurations (e.g. light-light, dark-light, light-striped, etc. totaling 9 combinations) and observe how the change of clothes impacts the share of votes received by each image.

To simplify the notation below, we use capitalized two-letter codes for configurations of pairs and denote light-colored, dark-colored, and striped outfits by $L$, $D$, and $S$ respectively. With this noation, for example, $LD$ stands for a pair of a light-colored image from group 1  paired and a dark-colored image from group 2.

\subsection{Data} \label{subsec:pairwise data}
As mentioned above, we need to create a data set with similar pairs of images. For this purpose, we match the samples according to their estimated weight and height obtained for the images with the light-colored clothes.  The matching is performed by the same algorithm as in \Secref{sec:large} with the thresholds of $2 kg$ and $2 cm$, and leads to the total of 56 pairs. Thus, we create a set of pairs with persons that look similar when they both wear light-colored outfits. This set is the starting point of our analysis. 

\subsection{Crowdsourcing task setup} \label{subsec:pairwise crowdsourcing}
In this Mechanical Turk task, crowd workers see the pairs of images constructed in \Secref{subsec:pairwise data} one by one and have to decide who of the two shown people in each pair weights less. 
%We decided to keep our usual task size of 10 estimates and added 4 pairs of images twice (to obtain 60 pairs in total). 
We introduced duplicates in the tasks to use as a quality control measure for the collected votes. We expect the workers to stay consistent and vote for the same person twice. The results were quite promising, ca. 85\% of workers consistently chose the same image  in our experiments. 
%
To avoid random guesses, we embedded a two-letter code on each image. To give their vote, the workers had to enter the code on the chosen image into a single input field. In this way, the crowd workers have to actually look at the image (at least, to read the code) and can not randomly click on one of them. 

During the experiment, we ensured that all crowd workers see each pair in only one configuration. For example, when someone's task contained the $LL$ configuration of a pair, this worker would not see any of the remaining possible combinations with the same images and, thus, would not be biased by his previous knowledge. Furthermore, we created the tasks with mixed configurations, i.e. rather than collecting all results for $LL$ pairs first, we randomly chose the configuration of each pair in each task. 

In this manner, we conduct two experiments: one with light and dark-colored clothes, and another with light-colored and horizontally striped outfits. In both cases, we collected 40 votes for each pair of images, or a total of 19,200 votes (remember that in both experiments each pair appears in 4 different configurations) from 750 crowd workers.

\subsection{Analysis}  \label{subsec:pairwise analysis}

Our analysis in this section relies on the availability of multiple configurations for each pair. Let us consider the case of light- and dark-colored outfits. The analysis for light-colored and horizontally striped clothes is completely analogous.   

We can evaluate the difference between the light- and dark-colored outfits in our set by considering 4 different scenarios: $LL \rightarrow LD$, $LL \rightarrow DL$, $DL \rightarrow DD$, and $LD \rightarrow DD$. Each scenario represents a special transition between two configurations: in all cases, exactly one person changes from a light-colored into a dark-colored outfit. The associated change of the votes share for this person can be attributed to the change of their clothes color (once again, we can not fully eliminate a possibility of biases that workers may have, or inaccurate Photoshop edits, but we can claim that the change is largely caused by the difference in clothes among the groups). Thus, for each scenario we focus on the change of votes received by the person who changes from light into dark clothes. 
If votes are gained through this transition, we can claim that the dark color has a slimming effect (remember that the crowd workers vote for the person whose weight they believe to be slimmer, hence an increased number of votes indicates a change that contributes to a slimmer body image).

For example, when we consider the impact of the clothes color, we would expect that among the $LL$ pairs both images are chosen ca. 50\% of times (since we matched the images on this configuration). 
If dark clothes indeed have a slimming effect, we can expect that for the $DL$ case the votes shift towards the first person (and vice versa for the $LD$). Finally, the $DD$ configuration should be closer to the original $LL$ case than both other setups.

\subsection{Results}  \label{subsec:pairwise results}

%Finally, let us present the study results. 
We begin by evaluating the effect of color change and compare light- and dark-colored outfits. The distributions of votes on all pairs for 4 different configurations are summarized in \Tabref{tab:pairwise LD}. Each row- or column-wise transition in \Tabref{tab:pairwise LD} describes one possible scenario: e.g. going from the upper-left to the lower-left cell means that the first person in the pair changes their clothes from light into dark ($LL \rightarrow DL$) and wins 4.1\% of votes on average. The three other scenarios are analogous. Note how the share of votes changes according to our expectations described in the last paragraph of \Secref{subsec:pairwise analysis}. The distribution of the changes in votes shares caused by these transitions is shown in \Figref{fig:pairwise} (left) and summarized in the first row of \Tabref{tab:pairwise summary}. From the right-skewed distribution in \Figref{fig:pairwise} (left) we can conclude that the dark color has a small (on average, just 2.73\% of votes are gained by changing into dark) but statistically significant slimming effect on the weight perception. 

We perform the same analysis for the case of light-colored and horizontally striped clothes. The results are summarized in \Tabref{tab:pairwise LS}, \Figref{fig:pairwise} (right) and \Tabref{tab:pairwise summary}. Overall, the pairwise comparison clearly indicates that there is no significant difference between these two types of clothes. 

\begin{table}
\centering
	\caption{Share of votes for the first person in each pair (with the 95\% confidence interval). Each pair appears in 4 different configuration: light-light ($L_1,L_2$), light-dark ($L_1,D_2$), dark-light ($D_1,L_2$), and dark-dark ($D_1,D_2$).}
	\label{tab:pairwise LD}
	\begin{tabular}{l | c | c}
		    & $L_2$ & $D_2$ \\
		 \hline
		$L_1$ & 52.5\% (46.7\%, 58.2\%) & 51.1\% (44.7\%, 57.6\%)\\
		\hline
		$D_1$ & 56.6\% (50.7\%, 62.8\%) & 54.8\% (48.3\%, 61.5\%) \\	 
	\end{tabular}
\end{table}


\begin{figure}
    \centering
	\begin{subfigure}{.48\columnwidth}
 		\centering
  		\includegraphics[width=\linewidth]{Plots/plot_pairs_results1_on_1.pdf}
	\end{subfigure}%
	\begin{subfigure}{.48\columnwidth}
  		\centering
  		\includegraphics[width=\linewidth]{Plots/plot_pairs_results_stripes1_on_1.pdf}
  	\end{subfigure}
	\caption{Share of votes gained by changing the outfit from light- into dark-colored (left) and from light-colored into horizontally striped (right).}
	\label{fig:pairwise}
\end{figure}


\begin{table}
\centering
    \caption{Percentage of votes for the first person in each pair (with the 95\% confidence interval). Each pair appears in 4 different variants: light/light ($L_1,L_2$), light/stripes ($L_1,S_2$), stripes/light ($S_1,L_2$) and stripes/stripes ($S_1,S_2$).}
    \label{tab:pairwise LS}
	\begin{tabular}{l | c | c}
		    & $L_2$ & $S_2$ \\
		 \hline
		$L_1$ & 0.513 (0.454, 0.574) & 0.536 (0.470, 0.604)\\
		\hline
		$S_1$ & 0.537 (0.475, 0.601) & 0.549 (0.476, 0.620) \\	  
	\end{tabular}
\end{table}


\begin{table*}
\centering
    \caption{Change of vote distribution (with 95\% confidence interval) and $p-$values of the Wilcoxon's test for two different scenarios in which people change their clothes.}
    \label{tab:pairwise summary}
	\begin{tabular}{ c | c | c | c | c}
	Changing from  & Changing to & Mean gain of votes [\%] with 95\% CI & $p-$value \\
	\hline			
	Light & Dark & 2.73, (0.88, 4.60) & 0.0069 \\
	Light & Stripes & 0.044, (-2.01, 2.07) & 0.58 \\
	\end{tabular}
\end{table*}

\section{Conclusion}

%\todo[inline]{Just a few words here, needs to be completed.}

\xhdr{Summary}
%
In this work, we tried to study the effects of clothing color (dark vs. light) and design (stripes) on perceived weight. We tried to, for the first time, answer the popular fashion claims surrounding these phenomena at scale and quantify the effective differences in weight perception.
We obtained a sense of perception through crowd sourcing, thus enabling us to scale our experiments to an order of magnitude bigger than previous studies in this area.
We started by creating a dataset of hundreds of images from Reddit posts in a weight lost forum. 
To mitigate the potential unobservable effects in this dataset, we created a smaller yet `cleaner' dataset of images edited using Photoshop.
%images. on various covariates such as height and weight.
We present three crowd sourcing studies on these two different data sets and conclude that:
\begin{itemize}
\item Dark color has a slight slimming effect in comparison to light-colored or horizontally striped clothes and, on average, visually `reduces' the weight of a person by ca. $2 kg$. Given the small difference, people are not very likely to notice it: if you change into dark clothes, others are only ca. $2.5\%$ likely to notice that your body image all of a sudden appears slimmer. 
\item We settle the long on-going debate about the effects of wearing horizontal stripes~\cite{feldon2000,swami2012,thompson2011}.
We can conclude that wearing horizontally striped or light colored clothes does not change the perception of your weight.
%whether you wear light or horizontally stripped clothes, others are likely to perceive your weight in the same way. 
\end{itemize}

%These conclusions are statistically significant and apply to both data sets. 
We note that the consistency of the results across the datasets makes our observations stronger, because each data has its own set of interesting properties.% on its own each data set has potential flaws.
%
The set of original Reddit images contains many unmeasurable covariates (e.g. different poses, backgrounds, clothes design or just inaccurate weight/height information provided by some users), and the results on this set could be attributed to these artifacts. On the other hand, all images of the edited set were processed by the same graphical designer and, thus, can be subject to the some repeating minor flaws, appear unrealistic or, as we observed in some cases, be inaccurately edited. Thus, the similarity of the results on both sets provides a much stronger ground for our conclusions. 

%We can briefly summarized the obtained results as:
%\begin{itemize}
%    \item Dark color has a slight slimming effect in comparison to light-colored or horizontally striped clothes and, on average, visually "reduces" the weight by ca. $2 kg$. Given the small difference, people are not very likely to notice it: if you change into dark clothes, the others are only ca. $2.5\%$ likely to notice that your body image all of a sudden appears slimmer. 
%    \item The rumors about horizontal stripes are not justified in our studies. We can conclude that whether you wear a light or a horizontally stripped clothes, the others are likely to perceive your weight in the same way. 
%\end{itemize}`

Our results not only provide a solid empirical ground for everyday fashion advice, but also have other applications. 
Our work provides technical advances in automatic pattern detection (to identify stripes/color) with crowd sourcing techniques thus providing a scalable solution to studies interested in popular fashion perception.
Though each of these may not be novel in their own right, the applications of such methodology in the fashion industry could be numerous. 
Given the rise of deep learning driven fashion technologies~\cite{liu2016deepfashion} and the potential of AI designed clothes~\cite{zhu2017your}, such scalable methodolgies would be required to get a quick sense of how a large population would perceive clothing.
%and datasets could be useful in designing better clothing.

\xhdr{Limitations}
This work has several limitations.
Firstly, the datasets we consider are `small' (few hundred images) compared to traditional big data studies involving thousands of images. 
Given the potential confounds that arise from such `in the wild' images, we deliberately made the choice to keep the data set small to allow us to manually control for as many confounds as we can.
Second, as we briefly allude to in the discussion, there are many biases that arise in crowd sourcing. For instance, crowd workers judging images taken under different conditions could be subject to various biases.
We argue that this need not be a necessarily bad thing, as such biases are also common in the general perception of humans in the real world.
However, more care could be taken in selecting the crowd workers, so that they closely resemble the general audience for a fashion item.

%It is hard to obtain cleaner datasets. However, such results are important and interesting.

\xhdr{Future work}
The study provides interesting directions for future research in both crowd and data driven fashion design.
%
We do not answer \textit{what} makes people in darker clothes appear thinner. Though there were attempts to answer this using mathematical models~\cite{helmholtz1867,thompson2011}, there are studies contradict them. Asking a large crowd audience why they think an image appears slimmer could provide answers to such question.
Second, many large scale fashion datasets are being available~\cite{liu2016deepfashion,xiao2017fashion}. Due to the potential of our automated techniques for stripes and color detection, it would be possible to generalize our analysis much larger datasets. This could be interesting because the scale could help us eliminate a large source of possible biases.

\iffalse
\appendix
\section*{Appendix}
\section{Color classification} \label{sec:color classification}

As the first step to estimation of the impact of clothes color on weight perception, a systematic way to classify the clothes as dark- or light-colored (or possibly neutral) is required. In this section, we describe our approach that avoids tedious and, possibly, biased manual inspection.
%
When referring to the color or stripes in the clothing, we refer only to the upper-body clothing. 
This is not a weak assumption since we are interested in weight perception, and the upper body plays a significantly important role in this. 
This formulation also fits particularly well to the data set at hand because of many images that show only a person's torso and not their full body.   

Our approach to color detection relies on the PoseNet \cite{cao2016} for body pose recognition. 
PoseNet, given an image, identifies the approximate pose by identifying all joints and body parts.
Once the positions of all joints and body parts are localized, we can sample the $RGB$-values (in range $[0, 255]$) of the pixels along the main upper body line - from the neck to the underbelly. 
We define the resulting color of the outfit as the value mean of the three channels of all sampled pixels. 
In this way, every image can be assigned a single `brightness value' $bv$ with $0$ being perfect black and $255$ perfect white. 

We used the described algorithm to compute brightness values $bv$ for all images in the image set from Section \ref{subsec:large data}. We manually evaluated the algorithm on all a sample of 100 images in the dataset and it works perfectly. 
Fig. \ref{fig:color qunatiles} shows 4 sample images with the corresponding values $bv$.

\begin{figure}[ht]
  \centering
  \includegraphics[width=0.8\textwidth]{Plots/color_quantiles.pdf}
  \caption{Sample images with detected body line and computed brightness value ($bv$). The images are (from left to right) at 0th (the darkest), 33th, 66th and 100th (the brightest) percentile of $bv$.}
  \label{fig:color qunatiles}
\end{figure}


\section{Stripes detection} \label{sec:stripes detection}

To make grounded statements on the effect of horizontal stripes on slimness, a large number of samples with striped clothing is required. 
A relatively small size of the image set from \Secref{subsec:large data} lets us detect the relevant samples manually. However, it turns out that wearing horizontal stripes is rather uncommon (from  images from \Secref{subsec:large data} only ca. 35 are suitable). Thus, an automated approach for collection and processing of additional data is required.

Similar to the color classification in \Secref{sec:color classification}, our approach for stripes detection relies on the PoseNet for detection of the main upper body line. $RGB$ values are sampled along the detected line and a single value for each pixel is computed by averaging over three color channels. Then we process the sequence of sampled pixel-wise values by a median (of length 5) and a third-order Savgol filter, which smoothes the noise and undesired fluctuations. 
Finally, we apply a Fourier transform on the output of the filters. The amplitudes of the resulting Fourier coefficients of different frequencies are important: our experiments suggest that stripes on the clothes lead to a large coefficient of the frequency that corresponds to the actual number of visible stripes. 
Therefore, we make use of the following heuristic rule: classify as a positive example (striped) any outfit that has its maximal (in terms of amplitude) Fourier coefficient in the range $[6,25]$, corresponding to a typical number of visible stripes. 
\Figref{fig:stripes classifier} illustrates the method on an image that is classified as positive.

\begin{figure}
\centering
\begin{subfigure}{.24\textwidth}
  \centering
  \includegraphics[width=0.4\linewidth, clip=true, trim=50 10 100 10]{Plots/plot_stripes_sample.png}
  \caption{}
\end{subfigure}%
\begin{subfigure}{.24\textwidth}
  \centering
  \includegraphics[width=\linewidth]{Plots/plot_stripes_colorline.pdf}
  \caption{}
\end{subfigure}
\begin{subfigure}{.25\textwidth}
  \centering
  \includegraphics[width=\linewidth]{Plots/plot_stripes_colorline_smooth.pdf}
  \caption{}
\end{subfigure}
\begin{subfigure}{.25\textwidth}
  \centering
  \includegraphics[width=\linewidth]{Plots/plot_stripes_colorline_fourier.pdf}
  \caption{}
\end{subfigure}
\caption{Steps of the algorithm for stripes detection: identification of the main upper-body line (a), pixel-wise sampling of RGB values (mean subtracted) along the line (b), application of smoothing filters to the pixel-wise RGB values (c), and Fourier transform of the resulting sequence (d). The sample is classified as positive because of the magnitude of the 19-th Fourier coefficient (note that exactly 19 stripes are crossed by the main body line).}
\label{fig:stripes classifier}
\end{figure}

We should point out that the resulting algorithm relies on empirical observation and heuristics, so that the obtained results are far from perfect. In many cases other periodic variations of color (e.g. checkerboard patterns, letters, graphics or just different shading due to certain light conditions) trigger a positive response. Overall only ca. 20\% of the detected samples indeed wear horizontal stripes, and thus, manual inspection of the results is required to remove false positives. 
Nevertheless, the algorithm performs well for our purposes, as it provides a fast and simple way to detect striped clothes at scale. With this method we processed a dataset of almost 30,000 images from Reddit posts and obtained 90 images of people wearing clothes with horizontal stripes to the data set. 
\fi

